Through the Theory of Mind's Eye: Reading Minds with Multimodal Video Large Language Models

Can large multimodal models have a human-like ability for emotional and social reasoning, and if so, how does it work? Recent research has discovered emergent theory-of-mind (ToM) reasoning capabilities in large language models (LLMs). LLMs can reason about people's mental states by solving various text-based ToM tasks that ask questions about the actors' ToM (e.g., human belief, desire, intention). However, human reasoning in the wild is often grounded in dynamic scenes across time. Thus, we consider videos a new medium for examining spatio-temporal ToM reasoning ability. Specifically, we ask explicit probing questions about videos with abundant social and emotional reasoning content. We develop a pipeline for multimodal LLM for ToM reasoning using video and text. We also enable explicit ToM reasoning by retrieving key frames for answering a ToM question, which reveals how multimodal LLMs reason about ToM.

==> sections/benchmark.tex <==
\vspace{-0.1cm}
\section{Collaborative Agent Benchmark (\benchmarkname{})}
\vspace{-0.1cm}
% Despite the importance of effective multi-turn RL algorithms for building autonomous LLM agents, creating a realistic scalable benchmark that  evaluates different RL algorithms for LLM agents with reasoning-intensive tasks presents significant challenges. 
In this section, we first outline the foundational design principles of our \benchmarkname{} to address challenges in developing multi-turn RL algorithms for LLM agents, followed by a detailed explanation of the two specific tasks: %the specific setups for two tasks in \benchmarkname{} including 
Backend Programming and Frontend Design.

\vspace{-0.1cm}
\subsection{Design Principles}
\vspace{-0.1cm}
\textbf{(1) Sufficient task complexity that challenges the rea-
soning and generalization capability of agents.} As the ultimate goal is to enable the LLM agents to complete tasks on our behalf in the real world, where the agents need to address complicated challenges in out-of-distribution scenarios, it is essential that the benchmark reflects such realistic reasoning and generalization challenges. To achieve this, \benchmarkname{} is designed to align with realistic artifact creation tasks, where the objective of collaboration is to produce tangible outputs such as code or web pages. In order to do well, it is necessary for agents to dive deep into the structure of the code and nuanced differences in visual design for unseen requests and a potentially sub-optimal collaborator. 

%%YZ.1.28: might not have space for this
% As shown in the task example in Figure~\ref{fig:qualitative}, in order to arrive at the correct solution of python function, the agent not only needs to figure out what the intended python function is but also figures out what is right information to seek such as the concrete definition of ``symmetry'' and how to deal with corner cases like whether to include duplicate objects.
%%SL.1.26: This makes sense as a criterion, but the discussion here could be much more convincing as to why this criterion matters and how we fulfill it. E.g., consider giving some examples of the challenges the benchmark has
%%YZ.1.27: Get back to it after adding concrete qualitative examples in the appendix, but it might be 

\textbf{(2) Minimum %engineering
overhead for fast research prototyping.} To achieve this, we ground each collaboration task with the goal to re-create the exact same product as the reference artifact. In this way, the human collaborator can be easily simulated by an LLM with access to the reference artifact to faithfully answer the uncertainties from the LLM agent. Furthermore, the presence of a reference artifact allows \benchmarkname{} to employ objective and functional evaluation metrics that assess the similarity between the final collaborative product and the reference artifact. As a result, the only requirement needed for setting up \benchmarkname{} is API access for some LLM calls and some Python packages for running code and rendering HTML web pages. Although in real-world scenarios the human collaborator might only have a general idea of the desired final product, having access to a clear reference artifact is a reasonable assumption that significantly enhances reliability.

\textbf{(3) Sufficient task diversity for RL training without
overfitting.} As the best LLMs are often trained on a huge amount of data, it is essential that our benchmark contains enough tasks to understand the scalability of different multi-turn RL algorithms while at the same time ensuring the reliability of simulation and evaluation. Therefore, we designed \benchmarkname{} to be highly scalable, with more than 10k different procedurally-generated tasks, which also can be easily expanded as needed by incorporating more existing artifacts such as code and web pages. The difficulty of \benchmarkname{} can be easily adjusted 
%as well  as the base capability of LLMs increase 
by simply creating more collaboration tasks with more complicated code bases and web pages.

Next, we will describe detailed setups of \benchmarkname{}, including Backend Programming and Frontend Design.
%%SL.1.26: feels like we need some transition sentence after this to lead into the next subsection (eg next we'll describe the tasks)


% As the capabilities of LLM agents continue to advance, often reaching the limits of existing benchmarks, it is essential that improvements in these benchmarks translate directly to enhancements in real-world, production-scale scenarios. To achieve this, \benchmarkname{} is designed to align with realistic artifact creation tasks, where the objective of collaboration is to produce tangible outputs such as code or webpages. Consequently, advancements in \benchmarkname{} not only indicate a more collaborative LLM agent but also have a significant impact on real-world productivity, enhancing efficiency in artifact creation processes.
% %%SL.1.17: While it's ok to appeal to application-level relevance a little bit, it's more impotrant to explain to ML people why they should care about this (ML people probably don't care much about enhancing efficiency of artifact creation, but they care about core ML problems)

% \textbf{(2) Simulation and evaluation of tasks should be reliable.} Given the high costs associated with human supervision, it is essential to utilize LLMs to simulate the responses of human collaborators and to implement automatic evaluation metrics to enhance accessibility. This presents the challenge of using LLMs to reliably simulate human-like reactions and of evaluating free-form collaborations, especially since current LLMs may not excel in collaborative tasks. To address this, we have designed an asymmetric structure for \benchmarkname{}. In this setup, the human collaborator has access to a reference artifact, such as code and a webpage, while the agent collaborator must interact with the human collaborator to obtain information about the reference artifact. This approach simplifies the task for the human collaborator, making it more feasible to simulate reliably. Furthermore, the presence of a reference artifact allows \benchmarkname{} to employ objective and functional evaluation metrics that assess the similarity between the final collaborative product and the reference artifact. Although in real-world scenarios, the human collaborator might only have a general idea of the desired final product, having access to a clear reference artifact is a reasonable assumption that significantly enhances the benchmark's reliability.
% %%SL.1.17: I'm really struggling to understand this paragraph. Is it just saying that we have ground truth designs so that we can compute rewards? Feels like there should be a much simpler way to say it.

% \textbf{(3) Tasks should focus on the collaboration capability.} Finally, \benchmarkname{} is designed to specifically evaluate the collaboration capability of LLM agents. Only the human collaborator has access to the reference artifact and the evaluation is based on the similarity between the final product and the reference artifact. As the only way for the LLM agent to learn about the reference artifact is through collaborations with the human collaborator, it is impossible for even the strongest LLM agent to do well on its own and it has to learn nuanced collaborative behaviors in order to complete the tasks. 
% %%SL.1.17: why is focusing on collaboration capability important?

% %%SL.1.17: Generally, my sense is that the tasks are really cool, but the description and motivation of the tasks kind of undersells how interesting they are. I think tying the tasks to fundamental challenges in the design of LLM agents will make this section much more compelling.
\vspace{-0.1cm}
\subsection{Backend Programming Collaborations}
\vspace{-0.1cm}


\textbf{Task description.} In this task, the agent is required to collaborate with the human simulator to write a custom Python function (up to 50 lines). In the beginning of the collaboration, the agent is provided with a high-level description and the signature of the function. However, many concrete details, such as what conditions should be considered and what to do at edge cases, are not provided, and the agent has to reason and decide what clarifications are needed from the human simulator. The human simulator will provide a brief explanation in natural language to each clarification question based on the reference code visible only to the human simulator, but it will not write code. The interactions are limited to 10 back-and-forth rounds between the agent and the human simulator. The interaction ends either when the agent has decided to give the final solution or the maximum number of rounds has been reached. The success of the agent is evaluated by 10 hidden unit tests for each function for 0/1 reward only at the end of each collaboration.

\textbf{Data generation.} Python functions, high-level descriptions, and unit tests are generated by prompting Llama-3.1-70B-Instruct~\citep{dubey2024llama3herdmodels} to extract a python function as inspired by an Internet excerpt from DCLM~\citep{li2024datacomplmsearchgenerationtraining}. Only the tasks where the generated python functions can pass their corresponding unit tests are kept. We generate 10k such tasks in the train set and 1k tasks in the test set where tasks in the test set are manually inspected by authors. 15k offline train trajectories are generated by zero-shot prompting Llama-3.1-8B-Instruct as agent and Llama-3.1-70B-Instruct as human simulator.

\vspace{-0.1cm}
\subsection{Frontend Design Collaborations}
\vspace{-0.1cm}

\textbf{Task description.} In this task, the agent is required to collaborate with the human simulator to design a web page by writing an HTML snippet (around 100 lines). At the beginning of the collaboration, the agent is provided with a high-level description of the web page. Again, many concrete details such as the layout and color palette of the web page are missing and only visible to the human simulator. At each round, the agent has a chance to write an HTML solution and it will be rendered by the web browser. The human simulator will be able to examine the rendered web page from the agent and the reference web page, then describe their differences to the agent. Similar to the backend programming collaboration, the interaction ends either when the agent has decided to give the final solution or the maximum number of 10 rounds has been reached. The performance of the agent is evaluated by the cosine similarity of CLIP~\citep{radford2021learningtransferablevisualmodels} embeddings between the agent solution and reference web page, the best metric found in prior works~\citep{si2024design2codefarautomatingfrontend} for frontend design. It serves as a reward within the range of 0 to 1 only at the end of the collaboration.

\textbf{Data generation.} The tasks containing reference web pages and high-level descriptions are from WebSight~\citep{laurençon2024unlockingconversionwebscreenshots}. We include 10k such tasks for training and 500 for the test set. The test set tasks are manually inspected by the authors. We generate 6k offline train trajectories by zero-shot prompting Llama-3.1-8B as agent and Qwen2-VL-72B~\citep{yang2024qwen2technicalreport} as human simulator.

% Maybe put a table here summarizing the statistics of each task

% \begin{table}\centering
% \begin{adjustbox}{width=0.45\textwidth}
% \begin{tabular}{ c |c c c }
%  Task & Train Tasks & Trajectories &  Test Tasks \\ 
%  \midrule
%  \textbf{Backend Programming} & 10k & 20k  & 1k \\  
%  \textbf{Frontend Design} & 1k & 6k & 100
% \end{tabular}
% \end{adjustbox}
% \label{tab:task_statistics}
% \caption{Dataset statistics for tasks in \benchmarkname{}.}
% \end{table}
